Design Considerations and Robustness to Parameter Uncertainty in Wire-Wrapped Cam Mechanisms

Collaborative robots must simultaneously be safe enough to operate in close proximity to human operators and powerful enough to assist users in industrial tasks such as lifting heavy equipment. The requirement for safety necessitates that collaborative robots are designed with low-powered actuators. However, some industrial tasks may require the robot to have high payload capacity and/or long reach. For collaborative robot designs to be successful, they must find ways of addressing these conflicting design requirements. One promising strategy for navigating this tradeoff is through the use of static balancing mechanisms to offset the robot's self weight, thus enabling the selection of lower-powered actuators. In this paper, we introduce a novel, 2 degree of freedom static balancing mechanism based on spring-loaded, wire-wrapped cams. We also present an optimization-based cam design method that guarantees the cams stay convex, ensures the springs stay below their extensions limits, and minimizes sensitivity to unmodeled deviations from the nominal spring constant. Additionally, we present a model of the effect of friction between the wire and the cam. Lastly, we show experimentally that the torque generated by the cam mechanism matches the torque predicted in our modeling approach. Our results also suggest that the effects of wire-cam friction are significant for non-circular cams.

==> PaperFmt/preamble_algorithm.tex <==
\usepackage{algorithm,algorithmicx,algpseudocode}
%\usepackage{amssymb}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]} 

%\algrenewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1} %uncomment for black triangles

%%% example:
%\begin{algorithm}
%  \caption{Influx}
%  \label{influx}
%  \begin{algorithmic}[1]
%  \Input $p \in [0,1]$, $G$
%  \Output None \Comment{a test comment}
%  \For{$i = 0 \to 2^d-1$}\Comment{another test comment}
%    \If{$n(\nu_i) = 0$}
%      \If{ $x < p$}  \Comment{$x$ is a normal distribution number in the range of $[0,1]$}
%      \State Occupy $v_i$ site with probablility $p$
%      \EndIf
%    \EndIf
%  \EndFor
%  \end{algorithmic}
%\end{algorithm}

% for algorithmic package
%\renewcommand{\algorithmicxrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicxensure}{\textbf{Output:}}


==> tex_content/Two_DOF_Troque_friction.tex <==
\subsection{Two DOF Wire-Wrapped Cams}\label{sec:2dof_finite_friction}
For the two DOF cam system, we can easily adapt Eq. \eqref{eq:tau1_fric} for the torque on cam 1 from spring 1, $\bs{\tau}_{1,1}$, and the torque on cam 2 from spring 3, $\bs{\tau}_{2,3}$:
%
\begin{equation}\label{eq:tau_fric_2dof}
\begin{aligned}
  \bs{\tau}_{1,1} &= \bs{\tau}_{1,t} + \bs{\tau}_{2,s} \\
  \bs{\tau}_{2,3} &= \bs{\tau}_{2,t} + \bs{\tau}_{2,s}
\end{aligned}
\end{equation}
%
\noindent In this equation, $\bs{\tau}_{i,t}, i =1,2$ can be found by applying Eq. \eqref{eq:eta_t} to the correspond cam and $\bs{\tau}_{i,s}, i=1,2$ can be found by applying Eq. \eqref{eq:eta_s} to the corresponding cam. Now, Eq. \eqref{eq:tau_fric_2dof} can be used as a replacement for $\bs{\tau}_{1,1}$ and $\bs{\tau}_{2,3}$ in Eq. \eqref{eq:torque_2dof}. 

==> tex_content/convexity.tex <==
\subsection{Cam Convexity}\label{sec:conv}
In this section, we will derive the condition required to constrain the cam to be convex. Let $f\colon(a,b)\rightarrow\realfield{2}$ be a curve parameterized by $\phi\in(a,b)$ and $C(\phi) = (x(\phi),y(\phi))$ be a point on that curve. According to lemma 3.1.1 of \cite{Bajaj1991}, the curve (and therefore the cam) is convex if

\begin{equation}\label{eq:convex}
  x'(\phi)y''(\phi)-y'(\phi)x''(\phi) > 0
\end{equation}

\noindent For our purposes,

\begin{equation}\label{eq:xy_polar}
\begin{split}
  x(\phi) &= \rho(\phi)\cos(\phi)\\
  y(\phi) &= \rho(\phi)\sin(\phi)
\end{split}
\end{equation}

\noindent Therefore,

\begin{equation}\label{eq:xy_p_polar}
\begin{split}
  x'(\phi) &= \rho'(\phi)\cos(\phi)-\rho(\phi)\sin(\phi)\\
  y'(\phi) &= \rho'(\phi)\sin(\phi)+\rho(\phi)\cos(\phi)
\end{split}
\end{equation}

\noindent and

\begin{equation}\label{eq:xy_pp_polar}
\begin{split}
  x''(\phi) &= \rho''(\phi)\cos(\phi)-\rho(\phi)\cos(\phi)-2\rho'(\phi)\sin(\phi)\\
  y''(\phi) &= \rho''(\phi)\sin(\phi)-\rho(\phi)\sin(\phi)+2\rho'(\phi)\cos(\phi)
\end{split}
\end{equation}


\noindent Plugging (\ref{eq:xy_polar}-\ref{eq:xy_pp_polar}) into (\ref{eq:convex}) and simplifying yields

\begin{equation}\label{eq:convex_polar}
  \rho(\phi)^2+2\rho'(\phi)^2-\rho(\phi)\rho''(\rho) > 0
\end{equation}

\noindent This equation will be used to constrain the cam to be convex.

==> tex_content/friction.tex <==
\subsection{Cam Torque with Finite Friction: Two DOF}
For the two DOF cam system, we can easily adapt Eq. \eqref{eq:tau1_fric} for the torque on cam 1 from spring 1, $\bs{\tau}_{1,1}$, and the torque on cam 2 from spring 3, $\bs{\tau}_{2,3}$:
%
\begin{equation}\label{eq:tau_fric_2dof}
\begin{aligned}
  \bs{\tau}_{1,1} &= \bs{\tau}_{1,t} + \bs{\tau}_{1,s} \\
  \bs{\tau}_{2,3} &= \bs{\tau}_{2,t} + \bs{\tau}_{2,s}
\end{aligned}
\end{equation}
%
\noindent To find the torque the string applies to cam 1, $\bs{\tau}_{1,s}$, and to cam 2, $\bs{\tau}_{2,s}$, we can adapt Eq. \eqref{eq:tau_s}:
%
\begin{equation}
\begin{aligned}
\bs{\tau}_{1,s} &= \int_{0}^{\alpha_1}  \mb{r}_1(\sigma) \times -\mb{f}_1(\sigma) \; \text{d}\sigma \\
\bs{\tau}_{2,s} &= \int_{0}^{\alpha_2}  \mb{r}_2(\sigma) \times -\mb{f}_2(\sigma) \; \text{d}\sigma
\end{aligned}
\end{equation}
%
In this equation, the distributed force on cam 1, $\mb{f}_1(\phi_1)$, and on cam 2, $\mb{f}_2(\phi_2)$, can be found by adapting Eq. \eqref{eq:f_phi}:
%
\begin{equation}
\begin{aligned}
&-\mb{f}_1(\phi_1) = \\
&\frac{\tau_1(\alpha_1)e^{\mu_1\left(\phi_1 - \alpha_1  \right)}}{\| \mb{r}_1{'} \| }\left(  \mu_1\mb{r}_1{'} + \mb{r}_1{'}{'} - \mb{r}_1{'}(\mb{r}_1{'}\T\mb{r}_1{'})^{3}(\mb{r}_1{'}{'}\T\mb{r}_1{'}) \right) \\
&-\mb{f}_2(\phi_2) = \\
&\frac{\tau_2(\alpha_2)e^{\mu_2\left(\phi_2 - \alpha_2  \right)}}{\| \mb{r}_2{'} \| }\left(  \mu_2\mb{r}_2{'} + \mb{r}_2{'}{'} - \mb{r}_2{'}(\mb{r}_2{'}\T\mb{r}_2{'})^{3}(\mb{r}_2{'}{'}\T\mb{r}_2{'}) \right)
\end{aligned}
\end{equation}
%
\noindent To find the torque due to the force tangent to cam 1, $\bs{\tau}_{1,t}$, and to cam 2, $\bs{\tau}_{2,t}$, we can adapt Eq. \eqref{eq:tau_t}:
%
\begin{equation}
\begin{aligned}
\bs{\tau}_{1,t} &= \mb{r}_1(0) \times \tau_1(\alpha_1)e^{-\mu_1\alpha_1 }\frac{\mb{r}_1'(0)}{\| \mb{r}_1'(0) \|} \\
\bs{\tau}_{2,t} &= \mb{r}_2(0) \times \tau_2(\alpha_2)e^{-\mu_2\alpha_2 }\frac{\mb{r}_2'(0)}{\| \mb{r}_2'(0) \|}
\end{aligned}
\end{equation}
%
\noindent In the above equations, $\mu_1$ and $\mu_2$ are the static coefficients of friction between the cams and the string and:
%
\begin{equation}
\begin{aligned}
  \mb{r}_1(\phi_1) &= \rho_1(\phi_1)\begin{bmatrix}
             \cos(\phi_1) \\
             \sin(\phi_1)
           \end{bmatrix}\\
  \mb{r}_2(\phi_2) &= \rho_2(\phi_2)\begin{bmatrix}
             \cos(\phi_2) \\
             \sin(\phi_2)
           \end{bmatrix}
\end{aligned}
\end{equation}

Now, Eq. \eqref{eq:tau_fric_2dof} can be used as a replacement for $\bs{\tau}_{1,1}$ and $\bs{\tau}_{2,3}$ in Eq. \eqref{eq:tau1_2dof} and Eq. \eqref{eq:tau2_2dof}, respectively. 

==> tex_content/modal_and_convexity.tex <==
\section{Modal Cam Shape and Condition for Convexity}

==> tex_content/problem_statement.tex <==
\section{Optimization Based Wrapping Cam Design}
\subsection{Monomial Cam Basis}\label{sec:monomial}
%--------------------------------------------------
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{cam}
    \caption{Cam nomenclature}
    \label{fig:cam_terms}
\end{figure}
%-------------------------------------------------- 
As shown in Fig. \ref{fig:cam_terms}, we represent the profile of the cam using a polar function $\rho(\phi)$ where $\phi$ is a parameterizing angle along the cam. A monomial basis is used to represent $\rho(\phi)$ as shown in (\ref{eq:rho}). 
\begin{equation}\label{eq:rho}
  \rho(\phi) = \beta_n\phi^n+\beta_{n-1}\phi^{n-1}+\dots+\beta_{2}\phi^{2}+\beta_{1}\phi+\beta_0
\end{equation} 

\noindent For a given cam design (i.e. given $\rho(\phi)$, spring constant(s), etc.), we assume the torque on the cam $\tau$ as a function of cam angle $\theta$ can be found. In the following sections, we will define an objective function and constraints for the optimization routine that selects the cam monomial coefficients $\bs{\beta}\in\realfield{n}$, spring pre-extension(s) $\mb{x}_0$, and spring parameters $\mb{s}$ that minimize the difference between $\tau$ and the desired cam torque $\tau_d$. 

==> tex_content/springs.tex <==
\section{Spring Design}\label{app:spring}
\GJ{In this section $\tau$ is used for shear stress which conflicts with torque used earlier.} If the optimization routine were to directly select spring constant(s), it would be unclear how to select the corresponding maximum spring deflection constraints. Therefore, we will have the optimization routine select the spring wire diameter $d$ and spring outer coil diameter $D$. The spring constant $k$ and maximum allowable deflection $x_{max}$ will then be calculated using the selected spring geometry. The spring material shear modulus $G$, yield stress $\sigma_y$, and number of coils $N$ will be given as a specified design parameter. The resulting spring can be purchased from a custom spring supplier. If the user wants to select off the shelf spring(s), $d$, $D$, and $N$ can taken as inputs.

\subsection{Maximum Allowable Spring Deflection}
According to \cite{shigley}, the maximum shear stress $\tau$ experienced by a spring loaded with force $f$ is:
%
\begin{equation}\label{eq:shear}
  \tau = k_B\frac{8f\overline{D}}{\pi d^3}
\end{equation}
%
\noindent where $\overline{D} = D-d$ is the mean coil diameter and $k_b$ is the \textit{Bergstr\"asser factor}:
%
\begin{equation}\label{eq:kb}
  k_B = \frac{4c+2}{4c-3}
\end{equation}
%
\noindent and $c = \overline{D}/d$ is the \textit{spring index}. Now, the maximum allowable shear stress can be calculated using the material's yield stress $\sigma_y$ via the Tresca Criterion:
%
\begin{equation}\label{eq:tresca}
  \tau_y = \frac{\sigma_y}{2}
\end{equation}
%
\noindent Now plugging Eq. \eqref{eq:tresca} into Eq. \eqref{eq:shear} and solving for the applied force yields the maximum allowable force on the spring. This will later be used to calculate the maximum allowable deflection on the spring and subsequently used as a constraint:
%
\begin{equation}\label{eq:F_max}
  f_{max} = \frac{\pi d^3\sigma_y}{16n_sk_B\overline{D}}
\end{equation}
%
\noindent Where $n_s$ is a user specified safety factor.

Now, according to \cite{shigley}, the deflection of the spring as a function of the applied force is:
%
\begin{equation}\label{eq:def}
  x(f) = \frac{8f\overline{D}^3N}{d^4G}\left(1+\frac{1}{2c^2}\right)
\end{equation}
%
\noindent where $G$ is the shear modulus of the spring material. Plugging $f_{max}$ into Eq. \eqref{eq:def} yields the maximum allowable spring deflection:
%
\begin{equation}\label{eq:x_max}
  x_{max} = \frac{8f_{max}\overline{D}^3N}{d^4G}\left(1+\frac{1}{2c^2}\right)
\end{equation}
%
\subsection{Spring Constant}
Because the spring constant is the ratio of applied force to deflection $k = f/x$, the spring constant can be found using Eq. \eqref{eq:def}:
%
\begin{equation}\label{eq:k}
  k = \frac{d^4G}{8\overline{D}^3N}\left(1+\frac{1}{2c^2}\right)^{-1}
\end{equation}

